Recursive Self-Improvement LLM Agents for Inverter Dynamic Model Identification

This is a position paper. We demonstrate that recursive self-improvement (RSI) large language model (LLM) agents are a natural search engine for dynamic model identification of inverter-based resources (IBRs) whose internal controls are often proprietary and hidden from grid operators. White-box models provide physical transparency but require vendor disclosure; black-box models avoid this requirement but sacrifice interpretability; and existing grey-box approaches, including sparse and symbolic regression, are poorly suited to discovering feedback control architectures or incorporating control-engineering priors. Our position is that this gap can be alleviated by (1) restricting the search space to a typed vocabulary of standard control modules, including PI controllers, phase-locked loops (PLLs), low-pass filters, etc., composed under block-diagram grammar rules, and (2) using an RSI LLM agent to perform program search over candidate block-diagram models, guided by measured frequency-domain admittance data at the point of common coupling (PCC), while fitting the free parameters of each candidate by nonlinear least squares. We instantiate this position by adapting ThetaEvolve, an open-source program-evolution framework supporting in-context evolution and test-time learning, to inverter model discovery. In a proof-of-concept study on a grid-following (GFL) inverter benchmark, the RSI loop reduces the normalized root mean square error (NRMSE) of a naive open-loop model from 0.470 to 0.0435 and identifies a 15-module closed-loop structure that closely resembles the hidden ground-truth GFL controller.

==> method_old.tex <==
\section{Method: An RSI LLM Agent for Inverter Model Identification}
\label{sec:method}

% \todo{This section is a bit too long with 6 subsections and about 3.5 pages - which readers may have no patience to finish reading or feel lost. Is there a way that you can further break it down into two shorter sections so we can better review?}

We represent each candidate graph ${G}$ as a program that
instantiates modules and connects their ports. The identification
problem is then addressed by an iterative agentic loop that proposes a
structural edit, evaluates the resulting program against the measured
admittance, and uses the evaluation history to inform subsequent
proposals. Fig.~\ref{fig:approach} summarizes the resulting architecture.

Our implementation follows the evolutionary program-search framework of \textsc{ThetaEvolve} \cite{wang2025thetaevolve}. In addition to evolutionary search, \textsc{ThetaEvolve} supports reinforcement learning of the LLM proposal model during the search process, enabling recursive self-improvement through both model weights and accumulated context. We introduce three components tailored to inverter identification: a typed vocabulary of standard control modules together with an interconnection grammar (Section~\ref{sub:vocab}); a frequency-domain evaluator that returns both a scalar score and a structured residual record (Section~\ref{sub:eval}); and a proposal context that encodes control-engineering priors (Section~\ref{sub:prompt}). Sections~\ref{sub:rl} and \ref{sub:free} then describe two mechanisms by which the search loop can improve over time: updating the proposal policy through test-time reinforcement learning, or keeping the model weights fixed while accumulating information in the context. The former requires an open-weight model and local GPU resources, whereas the latter is training-free and is naturally suited to large off-the-shelf models accessed through an API.


\subsection{Search State and One Iteration}
\label{sub:state}

At iteration $t$, the search state is
\begin{equation}
\label{eq:state}
    s_t=(\mathcal{A}_t,\psi_t),
\end{equation}
where $\mathcal{A}_t$ is an archive of evaluated programs, their scores,
and evaluator diagnostics, and $\psi_t$ denotes the weights of the
proposal policy $\pi_{\psi_t}$. Each iteration consists of five steps.

\begin{enumerate}
\item \emph{Context assembly.} A parent program is sampled from
$\mathcal{A}_t$ and a context $c_t=\Phi(\mathcal{A}_t)$ is assembled
from the parent's evaluator record, the module
catalog and grammar, and the domain priors of
Section~\ref{sub:prompt} %\todo{wrong section reference}.

\item \emph{Proposal.} The policy generates a proposal
$d_t\sim\pi_{\psi_t}(\cdot\mid c_t)$, which is applied to the parent to
produce a candidate program and the corresponding graph
$\mathcal{G}_t$. In \textsc{ThetaEvolve}, proposals are represented as
localized diffs, so each iteration corresponds to an attributable
structural modification. When an off-the-shelf model is accessed
through an API, the same search loop can instead use full-program
rewrites as the proposal interface.

\item \emph{Validation.} $\mathcal{G}_t$ is checked against the grammar.
Invalid candidates receive a fixed low score and are returned
immediately, \emph{without} any parameter fitting.

\item \emph{Evaluation.} A valid candidate is fitted and scored as in
Section~\ref{sub:eval}, producing a scalar reward $\mathcal{R}_t$ and a structured
residual record $\rho_t$.

\item \emph{Insertion.} The evaluated candidate
$(\mathcal{G}_t,\mathcal{R}_t,\rho_t)$ is added to the archive.
\end{enumerate}

The search state evolves according to
\begin{equation}
\label{eq:recursion}
    \mathcal{A}_{t+1}
    =\mathcal{A}_t\cup\{(\mathcal{G}_t,\mathcal{R}_t,\rho_t)\},
    \qquad
    \psi_{t+1}=\mathcal{U}\big(\psi_t,\mathcal{B}_t\big),
\end{equation}
where $\mathcal{B}_t$ contains the context--proposal--reward tuples
collected since the previous policy update, and $\mathcal{U}$ denotes
either the identity map or a reinforcement-learning update.

Equation~\eqref{eq:recursion} separates two mechanisms for recursive
improvement. The archive update changes the information available to
subsequent proposals, allowing successful structures and diagnostic
feedback to accumulate in the proposal context. The policy update can
additionally modify the proposal distribution itself using rewards
obtained during the search. We refer to these mechanisms as recursion
in \emph{context space} and recursion in \emph{weight space},
respectively. Sections~\ref{sub:free} and \ref{sub:rl} instantiate
these two variants within the same search loop.

\subsection{Module Vocabulary and Interconnection Grammar}
\label{sub:vocab}

The vocabulary $\mathcal{M}$ consists of the $23$ typed module kinds
listed in Table~\ref{tab:vocab}. Each module kind specifies its input
and output ports and associated signal types, free parameters and their
admissible ranges, contribution to model order, and small-signal
frequency-domain realization. For example,
\begin{equation}
    M_{\rm PI}(s)=k_{\rm P}+\frac{k_{\rm I}}{s},
    \qquad
    M_{\rm LPF}(s)=\frac{\omega_\tc}{s+\omega_\tc},
\end{equation}
where $k_{\rm P}$ and $k_{\rm I}$ are PI gains and $\omega_\tc$ is the
cutoff frequency. The SRF-PLL module implements the linearization of
\eqref{eq:pll}, while the rotation modules implement
\eqref{eq:rotation} linearized about the fitted equilibrium angle.
Ports use three signal types: scalar, $dq$ vector, and power pair.

The vocabulary is deliberately compact and closed: the search constructs
candidate models by interconnecting predefined control elements rather
than introducing arbitrary dynamics. This restriction keeps each
candidate interpretable as a conventional block diagram. We further
distinguish \emph{template} modules, which represent components that
would normally appear in an engineering control schematic, from
\emph{residual} modules such as Pad\'e delays and notch filters, which
can capture dynamics not explained by the template structure. 
% Residual modules are tracked separately by the evaluator, making it possible to
% distinguish structural explanations from improvements obtained through
% additional unmodeled dynamics. The gain--Pad\'e branch discussed in
% Section~\ref{sec:results} is one such residual insertion.

\begin{table}[!t]
\caption{Typed Module Vocabulary $\mathcal{M}$}
\label{tab:vocab}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}p{0.22\columnwidth}p{0.60\columnwidth}c@{}}
\toprule
Class & Module kinds & Order \\
\midrule
Physical plant &
\texttt{LCL}, \texttt{LFilter} & $6$, $2$ \\
Dynamic control &
\texttt{PI}, \texttt{PI\_dq}, \texttt{LPF1}, \texttt{LPF1\_dq},
\texttt{Integrator} & $1$--$2$ \\
Synchronization &
\texttt{SRF\_PLL} & $2$ \\
Operating point &
\texttt{Rot\_v}, \texttt{Rot\_i}, \texttt{PQ\_calc} & $0$ \\
Static algebra &
\texttt{Gain}, \texttt{Gain\_dq}, \texttt{Negate}, \texttt{Negate\_dq},
\texttt{PackDQ}, \texttt{SliceD}, \texttt{SliceQ}, \texttt{JMul},
\texttt{ConstZero} & $0$ \\
Residual &
\texttt{Pade1}, \texttt{Pade1\_dq}, \texttt{Notch} & $1$--$2$ \\
\bottomrule
\end{tabular}
\end{table}

Candidate graphs are constrained by a typed interconnection grammar.
At the port level, every edge must connect type-compatible ports, and
each input port must be driven exactly once. Combining multiple signals
therefore requires an explicit multi-source connection, which the
evaluator realizes as a summation. All free parameters remain symbolic
during structure generation and are assigned numerical values only
during parameter fitting (evaluation phase). At the graph level, every required input port of each instantiated module must have a source, the graph must define the terminal-current output, it must contain an \texttt{LCL} or \texttt{LFilter} module, and its declared order must lie within $[\underline{n},\overline{n}]$. Grammar validation is performed before parameter fitting. By enforcing these constraints at the structural level, the search is restricted to candidate programs that admit a well-defined and physically meaningful evaluation.

% Grammar validation is performed before parameter fitting. The grammar also removes structurally degenerate solutions that
% may achieve a favorable scalar score while bypassing the intended
% control architecture. In particular, it prohibits direct feedthrough
% from the terminal-voltage input to the current output, which could
% otherwise reproduce a passive admittance without representing the
% underlying feedback law.
% \subsection{Module Vocabulary and Interconnection Grammar}
% \label{sub:vocab}

% The vocabulary $\mathcal{M}$ contains the $23$ typed module kinds listed
% in Table~\ref{tab:vocab}. Each kind declares its input and output ports
% with their signal types, its free parameters with admissible ranges, its
% contribution to the model order, and its small-signal frequency-domain
% realization. For example,
% \begin{equation}
%     M_{\rm PI}(s)=k_{\rm P}+\frac{k_{\rm I}}{s},
%     \qquad
%     M_{\rm LPF}(s)=\frac{\omega_\tc}{s+\omega_\tc},
% \end{equation}
% where $k_{\rm P}$ and $k_{\rm I}$ are PI gains and $\omega_\tc$ is a
% cutoff frequency, while the SRF-PLL module realizes the linearization of \eqref{eq:pll}
% and the rotation modules realize \eqref{eq:rotation} linearized at the
% fitted equilibrium angle. Three signal types are used: scalar,
% $dq$ vector, and power pair.

% Two aspects of Table~\ref{tab:vocab} are worth emphasizing. First, the
% vocabulary is closed and small: the search cannot invent a new dynamic
% element, only new \emph{interconnections} of recognizable ones, which is
% what makes every candidate readable as a block diagram. Second, the
% vocabulary separates \emph{template} modules, which correspond to
% components an engineer would name in a control schematic, from
% \emph{residual} modules (Pad\'e delays, notch), whose role is to absorb
% dynamics that the template layer does not explain. The evaluator counts
% residual modules separately, so a candidate that buys accuracy with
% unexplained dynamics is identifiable as such. The additional
% gain--Pad\'e branch reported in Section~\ref{sec:results} is exactly a
% residual-layer insertion of this kind.

% \begin{table}[!t]
% \caption{Typed Module Vocabulary $\mathcal{M}$}
% \label{tab:vocab}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{3pt}
% \begin{tabular}{@{}p{0.22\columnwidth}p{0.60\columnwidth}c@{}}
% \toprule
% Class & Module kinds & Order \\
% \midrule
% Physical plant &
% \texttt{LCL}, \texttt{LFilter} & $6$, $2$ \\
% Dynamic control &
% \texttt{PI}, \texttt{PI\_dq}, \texttt{LPF1}, \texttt{LPF1\_dq},
% \texttt{Integrator} & $1$--$2$ \\
% Synchronization &
% \texttt{SRF\_PLL} & $2$ \\
% Operating point &
% \texttt{Rot\_v}, \texttt{Rot\_i}, \texttt{PQ\_calc} & $0$ \\
% Static algebra &
% \texttt{Gain}, \texttt{Gain\_dq}, \texttt{Negate}, \texttt{Negate\_dq},
% \texttt{PackDQ}, \texttt{SliceD}, \texttt{SliceQ}, \texttt{JMul},
% \texttt{ConstZero} & $0$ \\
% Residual &
% \texttt{Pade1}, \texttt{Pade1\_dq}, \texttt{Notch} & $1$--$2$ \\
% \bottomrule
% \end{tabular}
% \end{table}

% A candidate graph must satisfy both port-level and graph-level
% constraints. Every edge connects an output port to a type-compatible
% input port; each input port is driven exactly once, so that combining
% several signals requires an explicit multi-source connection that the
% evaluator realizes as a summation; and every declared parameter is a
% symbolic placeholder rather than a number, since numerical values are
% owned by the fitting stage. At the graph level, all required ports and
% the external output must be connected, the PCC voltage input $v^{DQ}$
% must influence the model, the graph must contain a physical filter
% model, and the total declared order must lie in
% $[\underline{n},\overline{n}]$.

% Grammar violations are detected \emph{before} the evaluator is invoked.
% This is not merely defensive programming: parameter fitting dominates
% the cost of an iteration, so rejecting malformed candidates for free is
% what allows the loop to tolerate an aggressive proposal distribution.
% The grammar also excludes a specific failure mode that the scalar score
% would otherwise reward, namely wiring the terminal voltage input
% directly to the current output, which reproduces a passive admittance
% while bypassing the feedback law entirely.


\subsection{Frequency-Domain Evaluation and Structured Feedback}
\label{sub:eval}

For a grammar-valid structure $\mathcal{G}$, the evaluator assembles the
linear equations defined by the module transfer functions and their
interconnections. At each frequency $s=j\omega_k$, the system is solved
under unit perturbations along the two PCC-voltage axes, yielding the
predicted terminal admittance
\begin{equation}
Y_m(j\omega_k;\mathcal{G},\theta_m)\in\C^{2\times2}.
\end{equation}

\subsubsection{Parameter fitting}

For each operating point, the continuous parameters are obtained by
solving
\begin{equation}
\min_{\theta_m}\NRMSE_m(\mathcal{G},\theta_m).
\end{equation}
Although several individual modules are affine in their parameters, the
assembled admittance is generally a nonlinear rational function of
$\theta_m$ because the modules interact through feedback loops and
parameter-dependent transfer functions. The resulting least-squares
objective is therefore nonlinear and generally nonconvex, and may
contain multiple local minima. Reliable parameter fitting is important
because convergence to a poor local solution can make a plausible
structure appear inaccurate.

We use three measures to reduce this sensitivity. First, parameters are
optimized within bounds specified by their module types.
Second, each fit is initialized from a vector-fitting seed derived from
the measured response, together with a small number of Latin-hypercube
restarts. In our setup, this reduced the number of restarts required for
stable fitting from approximately twenty to five. Third, when the fit
at one operating point achieves an error below a prescribed threshold,
its solution is used to initialize the next operating point, reducing
the likelihood that an otherwise consistent structure is penalized by a
poor local minimum at a single operating condition.

% The residual weighting determines which parts of the admittance dominate
% the fit. Equal weighting of the four entries emphasizes the
% cross-coupling channels $Y_{dq}$ and $Y_{qd}$, where synchronization and
% decoupling dynamics are particularly visible. These channels, however,
% also have the lowest signal-to-noise ratio. In our experiments, equal
% entry-wise weighting led to substantial drift in the fitted PLL and
% power-loop gains. We therefore use a Frobenius residual at each
% frequency, allowing the larger diagonal channels to constrain the fitted
% parameters more strongly, while retaining entry-wise errors as
% diagnostic feedback to the proposal model.

% In the present proof of concept, the structure $\mathcal{G}$ is shared
% across the $M=2$ operating points
% $q^*\in{+0.3,-0.3}$ p.u., while the continuous parameters $\theta_m$
% are fitted independently at each operating point. A candidate therefore
% receives a high score only if the same block-diagram topology explains
% the measured admittance under both operating conditions.

\subsubsection{Reward}
The scalar reward supplied to the loop is
\begin{equation}
\label{eq:reward}
    \mathcal{R}(\mathcal{G})
    =
    -\log\!\left(
        \frac{1}{M}\sum_{m=1}^{M}
        \NRMSE_m
        +10^{-8}
    \right),
\end{equation}
The logarithmic transformation increases resolution among candidates in
the low-error regime, where differences in raw NRMSE become small.
Invalid, non-executing, or timed-out candidates receive fixed negative
scores below those assigned to valid candidates. Structural complexity is not included directly in
\eqref{eq:reward}. In the reported experiments, it is controlled through
the hard model-order bound. This avoids introducing an
additional scalar tradeoff between fitting accuracy and model
complexity.

\subsubsection{Structured feedback}
Alongside $\mathcal{R}$, the evaluator returns a record $\rho$ that is attached
verbatim to the next prompt. It reports the error resolved along three
axes: by frequency band ($5$--$50$\,Hz, $50$--$500$\,Hz,
$0.5$--$2$\,kHz, $2$--$5$\,kHz), by admittance entry ($Y_{dd}$,
$Y_{dq}$, $Y_{qd}$, $Y_{qq}$), and by operating point; it also reports
the module count, declared order, number of residual-layer modules, and
number of free parameters. This record is what converts a black-box
score into a diagnosis. 
% A scalar error tells the proposer only that a
% candidate is wrong; a residual concentrated below $50$\,Hz on the
% diagonal entries, with the two operating points disagreeing, is close to
% a statement about \emph{which control layer} is missing.


\subsection{Proposal Context and Control-Engineering Priors}
\label{sub:prompt}

The proposal policy does not operate on the scalar reward alone. Each
context $c_t$ contains four elements: the identification objective and
evaluation metric; the graph-construction API and module vocabulary of
Table~\ref{tab:vocab}; the parent program and its structured evaluator
record $\rho$; and control-engineering priors that guide the
interpretation of the residual.

A central prior is the relation between frequency scale and control
layer. GFL inverters typically contain synchronization, outer power
control, and inner current control loops with distinct bandwidths.
Consequently, residuals concentrated at low frequencies may indicate
missing or inaccurate synchronization or outer-loop dynamics, whereas
high-frequency residuals are more likely to involve the inner current
loop or filter dynamics. These cues encode generic knowledge of GFL
control architectures, allowing the proposer to use the frequency structure of the residual.

Two additional design choices determine how this information is used.
First, the requested edit scale is sampled at each iteration from three
tiers: parameter sharing or rewiring, single-module substitution, and
replacement of a plant component or complete control sub-loop, with
probabilities $0.3/0.4/0.3$. The mixture allows both local refinement
and larger structural changes while retaining the localized diff
representation used by \textsc{ThetaEvolve}. Second, in the reported configuration, the context contains only the sampled parent and its evaluator record, rather than multiple candidate programs. Population-level information therefore enters primarily through parent selection and the archive. This design reflects the limited context capacity of the open-source model used in our experiments and is less restrictive for recent commercial models with substantially larger context windows.

The control-engineering priors are specified independently of the
measurements from the target device. We include only knowledge that
could be stated before observing its admittance data, such as the
typical ordering of control-loop bandwidths and standard GFL control
components. A shortened excerpt of the context used in our experiments is
shown below.

\begin{tcolorbox}[
colback=gray!6,
colframe=gray!40,
boxrule=0.4pt,
arc=1.5mm,
left=1.5mm,
right=1.5mm,
top=1.3mm,
bottom=1.3mm,
title={\scriptsize\textbf{Context excerpt}},
fonttitle=\scriptsize
]
\scriptsize
\textbf{Task.} Evolve \texttt{build\_gfl\_skeleton()} to recover an interpretable small-signal GFL inverter model from measured PCC admittance $Y(j\omega)$.

\medskip
\textbf{Search space.}
Construct the model using only the provided typed control modules and
the graph API. All connections must satisfy the interconnection grammar;
module parameters remain symbolic and are fitted by the evaluator.

\medskip
\textbf{Evaluation.}
The evaluator fits the module parameters and returns the NRMSE averaged
over two operating points, together with errors resolved by frequency
band, admittance entry, and operating point. Lower NRMSE corresponds to
higher reward.

\medskip
\textbf{Domain cues.}
A GFL inverter typically contains synchronization, outer power control,
and inner current control loops with separated bandwidths. Use the
frequency distribution of the residual to identify which control layer
may be missing or incorrectly represented before proposing an edit.
If adding an expected control layer degrades the fit, examine its
feedback sign, measurement filtering, and injection point before
removing it.
\end{tcolorbox}


\subsection{Program Archive}
\label{sub:archive}

Both recursion variants use the same program archive $\mathcal{A}_t$ to
maintain evaluated candidates and select parents for subsequent proposals.
The archive contains a capped population of $P=10{,}000$ programs divided
among $I=10$ islands arranged in a ring, together with a global elite set
containing the $200$ highest-scoring programs found so far. Search proceeds
over the islands in round-robin order. Parents are sampled from a mixture
that favors strong candidates while preserving exploration: with probability
$0.6$ from the elite set, $0.2$ from the active island, and $0.2$ from the
full population. After approximately $1{,}000$ admitted programs, corresponding
to one full sweep of the $10$-island ring, each island shares its top
$10\%$ of programs with its two neighboring islands
\cite{novikov2025alphaevolve}. When the population cap is
reached, low-scoring programs are evicted. This design combines exploitation
of high-performing structures and occasional
global exploration.

\subsection{Recursion in Weight Space: Test-Time RL Post-Training}
\label{sub:rl}

Weight-space recursion updates the proposal policy during search using the
same evaluator reward used to rank candidate programs. This makes the update $\mathcal{U}$ in \eqref{eq:recursion} nontrivial,
allowing the policy to learn from evaluator feedback during search. The
policy can both suppress recurring failure modes, such as invalid edits
or incorrect use of the graph API, and improve its search strategy by
increasing the probability of structural edits that produce
higher-quality candidates. Thus, test-time RL can improve both proposal
validity and search efficiency without additional supervision
\cite{wang2025thetaevolve,yuksekgonul2026learning}.

\subsubsection{Update rule}

For each context $c_t$, the policy generates a group of $G$ independent
proposals $d^{(1)},\ldots,d^{(G)}$, each of which is evaluated to obtain
a reward $\mathcal{R}^{(i)}$. We use a group-relative policy-gradient
update (GRPO) \cite{shao2024deepseekmath,wang2025thetaevolve}, with rollout
advantages normalized within each group:
\begin{equation}
\label{eq:grpo}
\hat{A}^{(i)}
=
\frac{\mathcal{R}^{(i)}-\mu_c}{\sigma_c+\epsilon},
\qquad
\mu_c=\frac{1}{G}\sum_j \mathcal{R}^{(j)},
\end{equation}
where $\sigma_c$ is the group standard deviation and
$\epsilon=10^{-6}$. This group baseline avoids training a separate value
function and is well suited to the sparse, evaluator-driven feedback.

The normalized advantages are used in a clipped policy-gradient
objective, with truncated importance sampling to account for the
separation between the serving and training backends. In
experiments, each update uses $G=16$ rollouts for each of $32$ contexts,
giving $512$ evaluated proposals per rollout batch, followed by one
gradient step with learning rate $10^{-6}$. Generation reserves a
reasoning budget before requiring the model to emit an executable edit,
ensuring that every completed rollout produces a candidate that can be
evaluated.

\subsubsection{Reward shaping}

Group-relative normalization makes the update sensitive to the
\emph{relative} quality of proposals generated from the same parent.
Early in search, the largest reward differences often separate valid
from invalid edits, so weight updates primarily improve proposal
validity and compliance with the graph API. As the fraction of valid
proposals increases, the same mechanism increasingly distinguishes
among alternative structural edits. Groups whose rollouts receive
identical rewards contribute no gradient.

A second issue is parent reproduction: a policy can obtain the parent's
score without making a meaningful change. We therefore assign a fixed
penalty of $-0.3$ when the applied edit leaves the program unchanged.
% Our implementation also supports rewards defined relative to the parent,
% for example,
% \begin{equation}
% \Delta\mathcal{R}
% =
% \mathcal{R}(\mathcal{G}{\rm child})
% -
% \mathcal{R}(\mathcal{G}{\rm parent}),
% \end{equation}
% which directly rewards structural improvement. The experiments in
% Section~\ref{sec:results} use the absolute reward
% \eqref{eq:reward} together with the parent-reproduction penalty.

\subsubsection{When this option is appropriate}

Weight-space recursion requires an open-weight model, a training stack,
and GPU resources during search; our experiments use an $8$B-class
open-weight reasoning model. It also permits the identification pipeline
to remain on premises, which can be important for proprietary inverter
measurements. 
% More broadly, the updated policy can be retained across
% identification runs, allowing experience acquired on one search to
% inform subsequent searches.


\subsection{Recursion in Context Space: Training-Free Search with Large
Off-the-Shelf Models}
\label{sub:free} 

Context-space recursion is built into the search loop itself. As
evaluated programs and their structured feedback accumulate in the
archive $\mathcal{A}_t$, they change the information available to later
proposals. In the open-weight setting of Section~\ref{sub:rl}, this
contextual adaptation operates alongside the reinforcement-learning
updates to the proposal policy.

It can also operate on its own by setting
$\mathcal{U}=\mathrm{id}$ in \eqref{eq:recursion}. The proposal weights
then remain fixed, and improvement is carried entirely by the evolving
archive and the information assembled into the proposal context. This
configuration is particularly natural for large commercial models
accessed through an API, where model weights are unavailable but
closed-loop interaction with the evaluator remains possible. We do not
evaluate this standalone configuration in the present work and therefore
make no claim about its relative efficiency.

\subsubsection{Closed-loop agentic variant}

A stronger form of context-space recursion is to place a large coding
agent in a closed loop with the evaluator, following the emerging
autonomous-research paradigm \cite{karpathy2026autoresearch}. Compared
with single-shot proposal generation, this interface offers several
practical advantages. The agent can inspect and modify the full program,
execute the evaluator, detect invalid edits or implementation bugs, and
repair them before continuing the search. Larger commercial models also
provide substantially longer context windows, allowing the prompt to
carry richer domain knowledge and a longer history of previous attempts.
Their stronger reasoning and tool-use capabilities further support
multi-step workflows in which the agent formulates a structural
hypothesis, tests it, inspects the resulting diagnostics, and revises
the program within the same attempt. Recent work on such agentic
research loops has also highlighted design questions including how much
work an agent should perform before evaluation, how to isolate the
evaluator from the agent, and how to prevent optimization of the harness
itself rather than the underlying task
\cite{hogan2026alphalab,ishibashi2026harness}.

The main limitations are operational. When the agent is accessed through
a commercial API, measured admittance data, candidate models, and
potentially proprietary information about the device may leave the local
computing environment, which can be unacceptable in industrial
identification settings. API-based search also introduces inference
cost, latency, and dependence on a model whose weights and serving
behavior are outside the user's control. These trade-offs make the
agentic variant attractive when reasoning capability, tool use, and
rapid deployment are prioritized, while the open-weight configuration
of Section~\ref{sub:rl} is better suited to settings that require data
locality, reproducibility, or weight-space adaptation.

% For inverter identification, such a variant naturally suggests several
% additional safeguards. First, the context can describe multiple
% converter families---droop-forming, grid-following, hybrid, and
% virtual-synchronous---at comparable levels of detail to avoid biasing
% the search toward a particular architecture. Second, hardware
% parameters can be shared across operating points while
% equilibrium-dependent quantities are allowed to vary, with held-out
% operating points evaluated using the shared hardware parameters. This
% provides a direct test of whether a candidate represents a consistent
% physical device across operating conditions. Third, parameter
% identifiability can be reported alongside fitting error, helping
% distinguish well-supported modules from additional structure whose
% parameters are weakly constrained by the measurements. These extensions
% are motivated by the failure mode observed in
% Section~\ref{sec:results}, where improved fitting accuracy did not
% necessarily imply a more accurate recovered structure. Their systematic
% evaluation is left for future work in Section~\ref{sec:conclusion}.

Table~\ref{tab:options} summarizes the two recursion channels and their
practical instantiations.

\begin{table}[!t]
\caption{Comparison of Weight-Space and Context-Space Recursion}
\label{tab:options}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}p{0.22\columnwidth}p{0.34\columnwidth}p{0.34\columnwidth}@{}}
\toprule
& Weight space & Context space \\
\midrule
Adaptation &
proposal policy $\psi$ &
archive, prompt, and search history \\

Model access &
requires open weights &
supports open-weight or API models \\

Update mechanism &
test-time RL &
context accumulation and agentic feedback \\

Compute &
training and inference &
inference only when used alone \\

Data locality &
can remain fully on premises &
depends on model deployment \\

Persistence &
reusable policy checkpoint &
persistent archive and written history \\

Role in search &
improves proposal distribution &
improves information available to proposals \\

Combination &
used together with context recursion &
can operate alone or with weight updates \\

Status here &
evaluated in Section~\ref{sec:results} &
used in all runs; agentic extension not evaluated \\
\bottomrule
\end{tabular}
\end{table}


\subsection{Search Configuration}
\label{sub:config}

The reported experiments use an $8$B-class open-weight reasoning model
as the proposal agent, with targeted diff-based edits rather than full
program rewrites, and with the test-time reinforcement-learning
component of \textsc{ThetaEvolve} enabled. The program database contains
$10$ islands with a total capacity of $10^4$ candidates and an elite
archive of $200$. Candidates
are evaluated in parallel with a per-candidate wall-clock cap, each fit
using a vector-fitting seed and five Latin-hypercube restarts per
operating point. The admissible order range is $[0,30]$. A target
average NRMSE of $0.05$ is declared to the evaluator as a stretch goal
but does not stop the run: the search proceeds to the iteration budget,
and the trajectory of Section~\ref{sec:results} keeps improving after
the target is first met.

Because the test-time learning component was enabled throughout, the
results of Section~\ref{sec:results} should be read as the behavior of
the complete loop; we do not attempt to attribute the outcome to
in-context evolution or to the policy update separately, and a
controlled ablation is left for future work.


% \begin{figure}[!t]
% \centering
% \begin{tikzpicture}[node distance=4mm]
%   \node[loopblk] (ps) {Prompt\\sampler};
%   \node[loopblk, right=of ps, fill=orange!12] (llm) {LLM\\agent};
%   \node[loopblk, right=of llm, fill=yellow!16] (ev)
%       {Evaluator\\{\tiny validate, fit, score}};
%   \node[loopblk, right=of ev, fill=green!10] (db)
%       {Program\\database};

%   \draw[sig] (ps) -- (llm);
%   \draw[sig] (llm) -- node[slbl, above]{edit} (ev);
%   \draw[sig] (ev) -- (db);
%   \draw[sig] (db.south)
%       -- ++(0,-3.5mm)
%       -| node[slbl, below, pos=0.25]{parents + scores}
%       (ps.south);

%   \coordinate (dbpad) at ($(db.south)+(0,-5mm)$);
%   \begin{scope}[on background layer]
%     \node[
%         draw=blue!30,
%         rounded corners=3pt,
%         fill=blue!4,
%         fit=(ps)(llm)(ev)(db)(dbpad),
%         inner sep=3pt
%     ] {};
%   \end{scope}
% \end{tikzpicture}
% \caption{LLM-driven inverter-discovery loop adapted from
% \textsc{ThetaEvolve} \cite{wang2025thetaevolve}. The LLM proposes
% structural edits, while a deterministic evaluator enforces the grammar,
% fits continuous parameters, and scores each candidate against measured
% PCC admittance data.}
% \label{fig:loop}
% \end{figure}


% \subsection{Module Vocabulary and Interconnection Grammar}

% The vocabulary $\mathcal{M}$ contains 23 typed modules representing
% standard components of inverter models. Each module specifies its input
% and output types, free parameters, dynamic order, and small-signal
% frequency-domain realization. The vocabulary includes basic dynamic
% blocks such as PI controllers, integrators, low-pass filters, gains, and
% delays; inverter-specific control blocks such as the SRF-PLL, droop
% control, and linearized PQ calculation; coordinate operations such as
% Park rotations and multiplication by $\Jmat$; and physical models such
% as LCL and L filters. For example,
% \begin{equation}
%     M_{\rm PI}(s)=K_P+\frac{K_I}{s},
%     \qquad
%     M_{\rm LPF}(s)=\frac{\omega_c}{s+\omega_c}.
% \end{equation}

% A candidate graph must satisfy both port-level and graph-level
% constraints. Every edge connects an output port to a type-compatible
% input port, each input is driven exactly once, and multiple signals are
% combined through explicit summation blocks. At the graph level, all
% required ports and the external output must be connected, the PCC
% voltage input $v^{DQ}$ must influence the model, and the graph must
% contain a physical filter model. Candidates that violate these rules
% are rejected before parameter fitting. The grammar therefore allows
% nontrivial feedback interconnections while preventing structurally
% invalid programs from consuming evaluation budget.


% \subsection{Frequency-Domain Evaluation}

% For a grammar-valid structure $\mathcal{G}$, the evaluator assembles the
% linear equations implied by its module transfer functions and signal
% connections. At each frequency $s=j\omega_k$, the resulting system is
% solved under a perturbation of the PCC voltage to obtain the predicted
% terminal admittance
% \[
%     Y_m(j\omega_k;\mathcal{G},\theta_m).
% \]

% In the present proof-of-concept, the graph structure $\mathcal{G}$ is
% shared across the $M=2$ operating points
% $q^*\in\{+0.3,-0.3\}$ p.u., while the continuous parameters
% $\theta_m$ are fitted independently at each operating point by nonlinear
% least squares. The structural score is the mean of the resulting
% frequency-domain errors in \eqref{eq:nrmse}. Thus, a candidate receives
% a high score only when the same block-diagram topology can explain the
% measured admittance under both operating conditions.

% The scalar reward supplied to the evolutionary loop is
% \begin{equation}
% \label{eq:reward}
%     R(\mathcal{G})
%     =
%     -\log\!\left(
%         \frac{1}{M}\sum_{m=1}^{M}
%         \NRMSE_m
%         +10^{-8}
%     \right),
% \end{equation}
% with evaluation terminated once the target error threshold is reached.
% Candidate structures are additionally restricted to a prescribed range
% of total dynamic order to discourage unnecessarily complex models.


% \subsection{Prompt Design and Domain Knowledge}

% The LLM does not search from the numerical score alone. Each prompt
% provides four forms of context: the identification objective and
% evaluation metric; the graph-construction API and module catalog;
% high-performing parent programs selected by \textsc{ThetaEvolve}; and
% control-engineering priors that guide structural modifications.

% In particular, the prompt describes the canonical hierarchy of GFL
% control, synchronization, outer power regulation, and inner current
% control, and provides qualitative frequency-domain cues linking model
% mismatch to candidate subsystems. For example, low-frequency error may
% indicate an incorrect outer-control structure, whereas higher-frequency
% mismatch is more strongly associated with the inner current loop or
% filter dynamics. These priors allow the LLM to use the shape of the
% frequency-response error to propose targeted structural edits rather
% than relying solely on unguided mutation.

% A shortened excerpt of the prompt used in our experiments is shown
% below.

% \begin{tcolorbox}[
%     colback=gray!6,
%     colframe=gray!40,
%     boxrule=0.4pt,
%     arc=1.5mm,
%     left=1.5mm,
%     right=1.5mm,
%     top=1.3mm,
%     bottom=1.3mm,
%     title={\scriptsize\textbf{Prompt excerpt}},
%     fonttitle=\scriptsize
% ]
% \scriptsize
% \textbf{Task.}
% Evolve \texttt{build\_gfl\_skeleton()} to recover an interpretable
% small-signal GFL inverter model from measured PCC admittance
% $Y(j\omega)$.

% \medskip
% \textbf{Search space.}
% Construct the model only from the provided typed control modules.
% All connections must satisfy the graph grammar.

% \medskip
% \textbf{Evaluation.}
% The evaluator fits module parameters and returns the NRMSE averaged over
% two operating points. Lower NRMSE gives higher reward.

% \medskip
% \textbf{Domain cues.}
% A GFL inverter typically contains synchronization, outer power control,
% and inner current control. Use the frequency dependence of the residual
% to diagnose missing or incorrect control layers before proposing an edit.
% \end{tcolorbox}


% \subsection{Search Configuration}
% \todo{This method part needs to be better developed, to explain how the recursive improvement was performed - including both the option of RL post-training for open-source models or training-free when using large off-the-shelf models}
% The reported experiments use an 8B-class open-weight reasoning model as
% the proposal agent and targeted diff-based edits rather than full
% program rewrites. The program database contains 10 islands with a total
% capacity of $10^4$ candidates; periodic migration allows high-performing
% programs to propagate between islands while maintaining structural
% diversity, following the island-model paradigm used in evolutionary
% program search \cite{novikov2025alphaevolve}.

% \textsc{ThetaEvolve} also supports reinforcement learning of the
% proposal policy from evaluator feedback during test-time search \cite{wang2025thetaevolve}. We enabled this component in the experiments reported here. Full analysis of the influence of test-time training is left for future investigation.

% We disable this component in the experiments
% reported here, so the results isolate the effect of LLM-guided
% evolutionary search with fixed model weights. Test-time learning is
% left for future investigation in Section~\ref{sec:conclusion}.


